Exploiting Entity BIO Tag Embeddings and Multi-task Learning for Relation Extraction with Imbalanced Data

In practical scenario, relation extraction needs to first identify entity pairs that have relation and then assign a correct relation class. However, the number of non-relation entity pairs in context (negative instances) usually far exceeds the others (positive instances), which negatively affects a model's performance. To mitigate this problem, we propose a multi-task architecture which jointly trains a model to perform relation identification with cross-entropy loss and relation classification with ranking loss. Meanwhile, we observe that a sentence may have multiple entities and relation mentions, and the patterns in which the entities appear in a sentence may contain useful semantic information that can be utilized to distinguish between positive and negative instances. Thus we further incorporate the embeddings of character-wise/word-wise BIO tag from the named entity recognition task into character/word embeddings to enrich the input representation. Experiment results show that our proposed approach can significantly improve the performance of a baseline model with more than 10% absolute increase in F1-score, and outperform the state-of-the-art models on ACE 2005 Chinese and English corpus. Moreover, BIO tag embeddings are particularly effective and can be used to improve other models as well.

==> Motivation.tex <==
\section{Background}\label{sec:back}

In this section, we will give a brief introduction of the ranking loss function.

\begin{figure}[!ht]
	\centering
	\includegraphics[scale=0.40]{t.png}
	\caption{The effect of ranking loss's parameters.}
	\label{t}
\end{figure}

Given the distributed representation of the sentence $r_x$, the network computes the score for class $c$ by the following equation:
\begin{equation}
s(x)_c=r_x[W^{classes}]_c
\end{equation}
where $W^{classes}$  is an embedding matrix to be learned, whose number of columns equals to the number of positive classes. $W^{classes}_c$ is the embedding of the class $c$, a column vector whose number of dimensions is equal to the size of $r_x$. 
The network is trained by minimizing a pairwise ranking loss function. For each instance, the input is a sentence $x$ with a correct class label $y^+$ and an incorrect one $y^-$. Let $s(x)_{y^+}$ and $s(x)_{y^-}$ be the scores for $y^+$ and $y^-$ respectively, the pairwise ranking loss is computed by the following equations:
\begin{equation}
L^+=log(1+exp(\gamma(m^+ - s(x)_{y^+})))
\end{equation}
\begin{equation}
L^-=log(1+exp(\gamma(m^- - s(x)_{y^-})))
\end{equation}

Where $m^+$ and $m^-$ are margins and $\gamma$ is a scaling factor. For class Other, $L^+$ is set to zero.Following \cite{santos2015classifying}, we choose the class with the highest score among all incorrect classes as the one to perform a training step.

So the ranking loss function can be denoted as: 
\begin{equation}
\begin{aligned}
L_{r}=log(1+exp(\gamma(m^+ - s(x)_{y^+})))\\
+ log(1+exp(\gamma(m^- - s(x)_{y^-})))
\end{aligned}
\end{equation}

In equation(2), $L^+$ decreases by scale $\gamma$ as the score $s(x)_{y^+}$ increases, and it is almost zero when $s(x)_{y^+} > m^+$ , which encourages the network to give scores greater than $m^+$ for the correct class. Similarly in equation(3), $L^-$ decreases by scale $\gamma$ as the score $s(x)_{y^-}$ decreases, and it is almost zero when $s(x)_{y^-} < -m^-$, which encourages the network to give scores smaller than $-m^-$ for the incorrect classes. For the class Other, only $L^-$ is calculated to penalize the incorrect prediction.

During prediction time, an instance is considered as the class Other if all the scores are less than 0, otherwise the class with the highest score is chosen as the prediction. We find that the number 0 is in fact a threshold for determining whether an instance belongs to the positive classes, denoted as the hyperparameter $\theta$. $\theta$ has another effect of controlling the precision and the recall. Obviously, as $\theta$ increases, the constraint that a relation belongs to a positive class is stricter, and more instances will be predicted as the class Other, which leads to a higher precision for positive classes and a smaller recall. On the contrary, as $\theta$ decreases, more instances will be predicted as the positive classes, which leads to a smaller precision and a higher recall. We conducted some experiments to verify this property, as shown in Fig\ref{t}.

%In this paper, we built a multi task and multi loss learning architecture which composed of two parts: 1) Using cross entropy to identify the given entity pair and its corresponding sentence is a positive instance or a negative instance, and then 2) Using ranking loss to classify the relation type of the input. Besides, we added BIO tag information of entities in sentence to the input data, which can enrich the representation of the input sentence. The experimental results showed that both BIO tag information and the new architecture can improve the performance obviously.


